Sampling-based Motion Planning for Active Multirotor System Identification

This paper reports on an algorithm for planning trajectories that allow a multirotor micro aerial vehicle (MAV) to quickly identify a set of unknown parameters. In many problems like self calibration or model parameter identification some states are only observable under a specific motion. These motions are often hard to find, especially for inexperienced users. Therefore, we consider system model identification in an active setting, where the vehicle autonomously decides what actions to take in order to quickly identify the model. Our algorithm approximates the belief dynamics of the system around a candidate trajectory using an extended Kalman filter (EKF). It uses sampling-based motion planning to explore the space of possible beliefs and find a maximally informative trajectory within a user-defined budget. We validate our method in simulation and on a real system showing the feasibility and repeatability of the proposed approach. Our planner creates trajectories which reduce model parameter convergence time and uncertainty by a factor of four.

==> chapters/experiments.tex <==
\section{Results}\label{sec:experiments}
In this section we present the evaluation of our planner.
We implemented it in C++ using the \ac{OMPL} \cite{ompl}.
First we demonstrate the parameter information prediction principle on two generic polynomial segments.
Then we show in simulation, that the planner is capable of generating repeatable and persistently exciting parameter estimation experiments.
Finally we present performance benchmarks and validate our pruning criteria in benchmarking experiments.
\subsection{Propagation Visualization}
\begin{figure}
\centering
\input{graphics/propagation.eps_tex}
\caption{Two different polynomial segments and the predicted moment of inertia covariance $\sigmainertia$ depicted as ellipsoids.
The right maneuver only gives information about the pitch inertia.
The left maneuver excites roll, pitch and yaw simultaneously and shrinks the parameter covariance in all directions.}
\label{fig:propagation}
\vspace{-6mm}
\end{figure}

Figure \ref{fig:propagation} shows two different maneuvers and its predicted moment of inertia uncertainty.
The identification experiment needs to excite the \ac{MAV} in all directions to make all its parameters observable.
The planner is able to make these decisions by predicting and evaluating the parameter covariance matrix $\sigmaparameter$.

Due to the problem design (\ref{eq:mav_dynamics}) the parameter covariance does not grow during \ac{EKF} prediction (\ref{eq:prior}).
During measurement updates (\ref{eq:posterior}), however, the parameter covariance matrix shrinks depending on the linearization point and thus the trajectory.
This makes the parameter covariance matrix monotonically decreasing.
\subsection{Simulation Results}
We use RotorS to simulate an AscTec Firefly hexacopter \cite{Furrer2016}.
The \ac{MAV} has a generic odometry sensor delivering position and attitude measurements at \SI{100}{\hertz} with noise appropriate to modern external tracking systems.
The planner assumes measurements for propagating its covariance at the same rate.
We confine the \ac{MAV} to a cube with \SI{2}{\metre} side length.
In total we run $100$ experiments with a flight time of \SI{30}{\second} while planning \SI{60}{\second} for each trajectory.
We setup the planner model with a uniformly sampled parameter guess which we spread $\pm 50\%$ around the ground truth value.
We use the same \ac{EKF} as in the planner to estimate the parameters from the measurement data.

For comparison we generated $100$ random experiments using the same polynomial sampling algorithm.
But instead of searching the trajectory with least parameter uncertainty, we pick the trajectory with most polynomial segments.
This ensures generation of dynamic experiments with a maximum number of maneuvers.
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{graphics/stat_summary_sim}
\caption{Statistical summary of $100$ simulated parameter estimation experiments:
median and $95\%$-percentiles for random and optimized trajectories.
The optimized trajectories lead to faster convergence.
On average, within only \SI{10}{\second} of flight data the parameter estimates for the optimal experiments converge.
Especially the strongly coupled parameters $\inertiaz$ and $\kmom$ converge quickly compared to the random trajectories.}
\label{fig:stat_summary}
\end{figure*}
Fig. \ref{fig:stat_summary} shows the statistical summary of our parameter estimates.
On average, all parameters are converged after only \SI{10}{\second} of flight time with our proposed planner.
This is faster than for random excitation.
Especially, the strongly coupled parameters $\inertiaz$ and $\kmom$ converge quickly.

The thrust constant $\kthr$ already converges at hovering.
The drag constant $\kdrag$ requires some movement but then converges quickly.
The moments of inertia in x- and y-direction requires rolling and pitching of the \ac{MAV}.
The planner makes sure of exciting both directions as demonstrated in Fig. \ref{fig:propagation}.
Finally, the planner even finds trajectories that excite the moment of inertia around yaw and the moment constant $\kmom$.
The Euler equations (\ref{eq:euler}) reveal that those two constants are strongly coupled.
The estimator can only distinguish them through the cross product between the angular velocities.
The planner typically takes care of this by exciting roll, pitch and yaw simultaneously (see Fig. \ref{fig:est_j_z}).

As Fig. \ref{fig:est_j_z}  also reveals, the planner usually generates trajectories as aggressive as possible, given the input feasibility constraints.
This gives the best signal to noise ratio and allows fitting a maximum number of informative maneuvers into the allowed budget.

The experiments have further shown that given the \ac{MAV} can follow the trajectory closely,
the predicted covariance coincides well with the covariance estimated in simulated identification experiments.
This indicates that the simplifications we made by linearizing around the nominal trajectory and modeling are modest.
\begin{figure}
\centering
\includegraphics{est_j_z}
\caption{A simulated typical experiment trajectory.
To distinguish the effects of $\inertiaz$ and $\kmom$, the \ac{MAV} rolls, pitches and yaws simultaneously.
The planner tends to generate trajectories as aggressive as possible.
Also the planner is able to predict the covariance closely as shown in the bottom plot for $\inertiaz$.}
\label{fig:est_j_z}
\vspace{-6mm}
\end{figure}

Fig. \ref{fig:stat_sigma} shows that our planner leads to smaller sigma bounds and better estimates for all parameters.
In particular this becomes relevant for the coupled, difficult to identify parameters.
But we can also determine the easy to identify parameters more confidence with our optimized trajectories.
\begin{figure}
\centering
\includegraphics{graphics/stat_sigma}
\caption{Final sigma bounds and \acp{RE} of the $100$ simulated parameter estimation experiments.
Our planner leads to smaller sigma bounds for all parameters compared to random trajectories.
Especially for the coupled parameters $\inertiaz$ and $\kmom$ we achieve smaller errors and less uncertainty.}
\label{fig:stat_sigma}
\vspace{-6mm}
\end{figure}
\subsection{Modular Pruning}
For demonstrating the usefulness of the modular pruning strategy (\ref{eq:compare}) we ran $100$ planner benchmarks using \ac{OMPL} \cite{omplbenchmark}.
Fig. \ref{fig:pruning} shows the growth of belief nodes for running the planner with and without pruning.
Without modular pruning the number of belief nodes grows rapidly.
This lets the planning progress come to a halt.
Propagating all neighboring beliefs during the algorithm's uniform cost search occupied the planner.
It slows down the graph growth rate and thus prevents progress in uncertainty reduction.

Modular pruning on the other hand leads to faster convergence, lower parameter uncertainties and less volatility.
The planner ignores candidate trajectories that are bad in the sense of cost, state and parameter uncertainty.
Due to the submodular optimization criterion (\ref{eq:dopt}) the planner may also ignore optimal solutions.
This makes us lose guarantees on asymptotical optimality for the sake of faster convergence \cite{Hollinger2014}.
\begin{figure}
\centering
\includegraphics{pruning_benchmark}
\caption{Benchmarking of $100$ planner runs.
The plot shows the median and $95\%$-percentile of the number of belief nodes and corresponding uncertainty over the planner runtime.
In general, modular pruning leads to faster convergence, smaller parameter uncertainty and less volatility.}
\label{fig:pruning}
\vspace{-6mm}
\end{figure}


==> chapters/params.tex <==
\begin{table}[b]
\begin{center}
\caption{Experiment setup: planner settings, noise levels, known and unknown parameter ground truth values.}
\label{tab:parameters}
\begin{tabular}{llccccc}
\toprule
parameter                  & unit                                                               & simulation                & real                    \\
\midrule
$\terminationtime$          & \si{\second}                                                      & \num{30.0}                & \num{240.0}             \\
$\segmenttimethreshold$     & \si{\second}                                                      & \multicolumn{2}{c}{\num{6.0}}                       \\
$\posworldmin$              & \si{\metre}                                                       & \multicolumn{2}{c}{\numlistvector{-1.5;-1.0;0.75}}  \\
$\posworldmax$              & \si{\metre}                                                       & \multicolumn{2}{c}{\numlistvector{1.5;1.0;1.75}}    \\
$\totalthrustmin$           & \si{\metre\per\square\second}                                     & \multicolumn{2}{c}{\num{4.91}}                      \\
$\totalthrustmax$           & \si{\metre\per\square\second}                                     & \multicolumn{2}{c}{\num{14.75}}                     \\
$\angvelbasemax$            & $\pi$\si{\radian\per\second}                                      & \multicolumn{2}{c}{\numlistvector{2.0;2.0;2.0}}     \\
$\yawdotmax$                & $\pi$\si{\radian\per\square\second}                               & \multicolumn{2}{c}{\num{1.0}}                       \\
\addlinespace
$\diag{\forcesnoisecov}$    & \num{e-6}\si{\square\kilogram\square\metre\per\second\tothe{4}}   & \multicolumn{2}{c}{\numlistvector{5.0;5.0;7.0e2}}   \\
$\diag{\momentsnoisecov}$   & \num{e-5}\si{\square\kilogram\metre\tothe{4}\per\second\tothe{4}} & \multicolumn{2}{c}{\numlistvector{1.0;1.0;5.0e-1}}  \\
$\diag{\posnoisecov}$       & \num{e-7}\si{\square\metre}                                       & \multicolumn{2}{c}{\numlistvector{2.5;2.5;2.5}}     \\
$\diag{\attnoisecov}$       & \num{e-6}\si{\square\radian}                                      & \multicolumn{2}{c}{\numlistvector{2.89;2.89;2.89}}  \\
\addlinespace
$\mass$                     & \si{\kilogram}                                                    & \multicolumn{2}{c}{\num{1.6776}}                     \\
$\motorlocationbase$        & \si{\metre}                                                       & \multicolumn{2}{c}{\numlistvector{0.2165;0.2165;0.022}} \\
\addlinespace
$\kthr$                     & \si{\kilogram\metre}                                              & \num[round-mode=places,round-precision=2, scientific-notation=true]{8.5486e-06}     & - \\
$\kdrag$                    & $1$                                                               & \num[round-mode=places,round-precision=2, scientific-notation=true]{1.76e-2}        & - \\
$\kmom$                     & \si{\kilogram\square\metre}                                       & \num[round-mode=places,round-precision=2, scientific-notation=true]{1.3677728e-07}  & - \\
$\inertiax$                 & \si{\kilogram\square\metre}                                       & \num[round-mode=places,round-precision=2, scientific-notation=true]{0.0355358}      & - \\
$\inertiay$                 & \si{\kilogram\square\metre}                                       & \num[round-mode=places,round-precision=2, scientific-notation=true]{0.0469168}      & - \\
$\inertiaz$                 & \si{\kilogram\square\metre}                                       & \num[round-mode=places,round-precision=2, scientific-notation=true]{0.0993824}      & - \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> chapters/propagation.tex <==
\section{\ac{MAV} Model and Covariance Propagation} \label{sec:propagation}
In this section we describe how we predict the parameter uncertainty during planning.

The key idea is to recover nominal states, measurements and inputs from a planned polynomial trajectory.
Given these, we drive an \ac{EKF} to simulate state and parameter estimation.
Due to its recursive characteristic, \ac{EKF} allows computationally efficient propagation.
Also it is suitable for robust model-based \ac{MAV} state estimation \cite{burri2015robust}.

The resulting posterior covariance matrix gives us a belief about the estimate convergence.
We wish to find a trajectory with minimum predicted parameter covariance (see Fig. \ref{fig:propagation}).
In section \ref{sec:planner} we use this covariance propagation to evaluate a graph of randomly sampled trajectories.
%TODO(rikba): How does converged EKF covariance relate to observability? Source?

In the following we derive the algorithm for predicting the \ac{EKF} propagation.
The covariance prediction along a candidate trajectory segment boils down to three steps:
\begin{enumerate}
\item sampling the nominal flat states from the candidate trajectory,
\item recovering the full nominal state, measurements and rotor speeds from the flat states,
\item driving the \ac{EKF} covariance prediction and update about the recovered states.
\end{enumerate}
\subsection{Conventions and Notations}
Fig. \ref{fig:hexa} shows the main coordinate systems:
the inertial frame $\worldframe$ and the body frame $\baseframe$.
Furthermore, every rotor has a local frame $\rotorframe$ located at the end of each arm with the $z$-axis perpendicular to the rotor.
Pre-scripts specify the frame in which we express a quantity in.
For example $_A \mat{r} _{BC}$ would refer to the vector from point $B$ to $C$ expressed in coordinate frame $A$.
We use the direction cosine matrix $\mat{C}_{BA}$ to express a rotation,
which transforms a vector expressed in $A$ to $B$, i.e., $_B \mat{r} = \mat{C}_{BA} {_A \mat{r}}$.
\subsection{Model}
\begin{figure}
\centering
\input{graphics/hexa.eps_tex}
\caption{Sketch of a hexacopter with the world-fixed frame $\worldframe$, body-fixed frame $\baseframe$ and the individual forces and moments acting on each rotor and the base.}
\label{fig:hexa}
\vspace{-6mm}
\end{figure}
Following \cite{mahony2012multirotor} and previous work \cite{burri2016identification} we present a simple \ac{MAV} model.
The major rotor effects acting on the \ac{MAV} body are thrust $\rotorthrust$, combined induced rotor drag and blade flapping forces $\rotordrag$ and drag induced moments $\rotormoment$.
Assuming all rotor planes $\rotorframe$ are perpendicular to the $\zbase$-orientation, these are:
\begin{align}
\rotorthrustscalar &= \kthr \rotorspeedsqr,~ \rotorthrust = \rotorthrustscalar \zbase, \\
\rotordrag &= - \rotorthrustscalar \begin{bmatrix}
\kdrag & 0 & 0 \\
0 & \kdrag & 0 \\
0 & 0 & 0
\end{bmatrix} \left( \velbase + \angvelbase \times \motorlocationbase \right), \\
\rotorforce &= \rotorthrust + \rotordrag + \forcesnoise, ~\forcesnoise \sim \mathcal{N}(\zero, \forcesnoisecov),  \\
\rotormoment &= -\epsilon_i \kmom \rotorspeedsqr \zbase + \momentsnoise, ~\momentsnoise \sim \mathcal{N}(\zero, \momentsnoisecov).
\end{align}%
We add normally distributed process noise $\forcesnoise$, $\momentsnoise$ to account for modeling errors and aerodynamic uncertainties.
The thrust constant $\kthr$, drag constant $\kdrag$ and moment constant $\kmom$ determine the major aerodynamic effects.

Summing up all rotor forces and moments, the translational and rotational dynamics are:
\begin{align}
\velbasedot &= \frac{1}{\mass} \sumrotors \rotorforce - \angvelbase \times \velbase - \rotinv \gravityworld, \label{eq:newton}\\
\angvelbasedot &= \Inertiainv \left( \sumrotors \left( \rotormoment + \motorlocationbase \times \rotorforce  \right) - \angvelbase \times \Inertia \angvelbase \right), \label{eq:euler}
\end{align}%
where $\gravityworld = [0 ~ 0 ~ \gravityscalar]^T$ is the gravitational acceleration.

We neglect motor dynamics and assume motor speed commands convert instantaneously to motor speeds $\rotorspeed = \rotorspeedcmd$.
Also do not consider higher order linear and angular velocity terms, linear and angular acceleration of propellers, angular acceleration of motors and friction torque due to rotational motion.
Furthermore we assume that the \ac{CoG} coincides with the geometric center in $xy$-direction and some known offset in $z$-direction.
We can measure the mass $\mass$ and motor location with respect to the \ac{CoG} $\motorlocationbase$.
The unknown parameters $\param$ are the aerodynamic coefficients and the moments of inertia $\Inertia = \diag{[\inertiax ~ \inertiay ~ \inertiaz]}$:
\begin{align}
\param = \begin{bmatrix} \kthr & \kdrag & \kmom & \inertiax & \inertiay & \inertiaz \end{bmatrix}^T,
~ \paramdot = \zero.
\end{align}%
The following kinematic relationships between position $\posworld$ and velocity $\velbase$
and attitude $\att$ and angular velocity $\angvelbase$ complete the full \ac{MAV} state dynamics.
\begin{align}
\posworlddot &= \rot \velbase, \\
\attdot &= \frac{1}{2} \Omega(\angvelbase) \otimes \att .
\end{align}%
Essentially $13$ time-varying states, $6$ unknown parameters and $\numrotors$
rotor rate inputs $\rotors = [\rotorspeedabrv_1 ~ \ldots ~ \rotorspeedabrv_\numrotors]^T$ describe the system.
\begin{align}
\fullstate &= \begin{bmatrix} \posworld^T & \velbase^T & \att^T & \angvelbase^T & \param^T \end{bmatrix}^T, \label{eq:states}\\
\inputs &= \rotors, \label{eq:inputs}\\
\processnoise &= \begin{bmatrix} \forcesnoise^T & \momentsnoise^T \end{bmatrix}^T, \\
\processnoise &\sim \mathcal{N}(\zero, \processnoisecov), ~ \processnoisecov = \diag{[\forcesnoisecov,~ \momentsnoisecov]}, \label{eq:process_noise}
\end{align}%
and
\begin{align}
\mat{f}(\fullstate, \inputs, \processnoise) &= \ddt \fullstate. \label{eq:mav_dynamics}
\end{align}%

\subsection{Measurements}
\acp{MAV} are typically provided with position and attitude measurements either through an external motion tracking system or fusing internal sensors with GPS\@.
This choice makes the system states observable and thus gives enough information for the \ac{EKF} to refine the covariances.
During planning we simulate the measurements along the nominal trajectory given by the candidate path segment.
\begin{align}
\measurementpos &= \posworld_k + \posnoise, ~ &\posnoise \sim \mathcal{N}(\zero, \posnoisecov), \\
\measurementatt &= \attdiscrete \otimes \attnoise, \\
\attnoise &= \begin{bmatrix}
1 & \frac{1}{2} \smallattnoise
\end{bmatrix}^T , &\smallattnoise \sim \mathcal{N}( \zero, \attnoisecov), \\
\measurement_k &= [ \measurementpos^T ~ \measurementatt^T ]^T,
\end{align}%
where $\posnoise$ and  $\attnoise$ account for small measurement errors in position or attitude.
\subsection{Error Dynamics}
Since the \ac{MAV} dynamics model (\ref{eq:mav_dynamics}) is nonlinear we linearize the state and measurement about the nominal state for covariance propagation.
\begin{align}
\Delta \fullstate &= \fullstate - \fullstatenominal, \label{eq:error_state}\\
\Delta \measurement &= \measurement - \measurementmat \fullstatenominal = \zero \label{eq:innovation}.
\end{align}%
Simulating maximum likelihood measurements lead to zero innovation in (\ref{eq:innovation}).
Following Weiss and Trawny and Roumeliotis \cite{weiss2012vision, Trawny2005} we derive the error state (\ref{eq:error_state}).
We calculate the difference for all states but the error quaternion $\rotsmall$,
which we approximate as a small angle rotation around the nominal state:
\begin{align}
\delta \att &= \attnominal^{-1} \otimes \att & \delta \att \approx \begin{bmatrix}
1 & \frac{1}{2} \rotsmall^T
\end{bmatrix}^T   .
\end{align}%
We derive the Jacobians of (\ref{eq:mav_dynamics}) and (\ref{eq:error_state}) analytically to obtain the discrete-time linear system:
\begin{align}
\Delta \fullstate_{k+1} &= \systemmat \Delta \fullstate_{k} + \processnoise_k ,  &&\processnoise_k \sim \mathcal{N}(\zero, \processnoisecovdiscrete), \label{eq:state}\\
\Delta \measurement_k &= \measurementmat {\Delta \fullstate}_k + \measurementnoise_k, &&\measurementnoise_k \sim \mathcal{N}( \zero, \measurementnoisecovdiscrete ),\label{eq:meas}\\
\measurementnoisecovdiscrete &= \diag{[\posnoisecov,\attnoisecov]}.
\end{align}%
Note that only the system matrix $\systemmat$ is time-dependent and linearized about the sampled nominal trajectory at every \ac{EKF} update step.
We can calculate it quickly since $\systemmat$ is sparse and consists only of small-dimensional matrix operations.
\subsection{Linearization Point} \label{sec:linearization_point}
As shown in \cite{mellinger2011minimum}, polynomial trajectory segments in the differentially flat space of position and yaw allow reconstructing the nominal full \ac{MAV} state (\ref{eq:states}).
His derivations rely on a simpler point mass model but hold in approximation.
\cite{achtelik2014motion} uses these to generate linearization points for an \ac{IMU} and gyro driven \ac{EKF} in \ac{RRBT} for \acp{MAV}.
Additionally to position and attitude information we need to reconstruct the nominal rotor speeds along the trajectory to linearize $\systemmat$ at every update step.

There exists a linear mapping $\mat{A}$ between total rotor thrusts $\totalthrust$ and torques $\torques$ and rotor speeds $\rotors$ which can be (pseudo-)inverted to obtain the rotor speeds.
\begin{align}
\begin{bmatrix}
 \torques^T & \totalthrust
\end{bmatrix}^T &=  \mat{A} \cdot \rotors^2, \label{eq:n_mapping}\\
\torques &= \Inertia \mat{\alpha} + \angvelbase \times \Inertia \angvelbase, \\
\totalthrust &= \mass ||\thrust||_2, & \thrust = \velworlddot + \gravityworld, \\
\rotors^2 &=  \mat{A}^\dagger \cdot \begin{bmatrix}
 \torques^T & \totalthrust \label{eq:ff_cmds}
\end{bmatrix}^T .
\end{align}%
$\mat{\alpha}$ is the angular acceleration and is a function of the flat states and its derivatives (\ref{eq:flat_state}), i.e., snap and yaw acceleration \cite{mellinger2011minimum}.
Thus for the rotor speed inputs to be continuous we require at least continuous snap ($\nth{10}$ order) position and continues yaw acceleration ($\nth{6}$ order) yaw polynomial trajectories.
\subsection{Propagation Law} \label{subsec:propagation_law}
The \ac{EKF} propagation law along a trajectory is then formulated using the standard \ac{EKF} equations:
\begin{align}
\sigmastate_{k|k-1} &= \systemmat \sigmastate_{k-1|k-1} \systemmat^T + \processnoisecovdiscrete, \label{eq:prior}\\
\mat{S}_k &= \measurementmat \sigmastate_{k|k-1} \measurementmat^T + \measurementnoisecovdiscrete, \\
\mat{K}_k &= \sigmastate_{k|k-1} \measurementmat^T \mat{S}_k^{-1}, \\
\sigmastate_{k|k} &= ( \identity - \mat{K}_k \measurementmat ) \sigmastate_{k|k-1}.\label{eq:posterior}
\end{align}%
Since we are assuming the \ac{MAV} to follow the trajectory closely
and reconstruct the approximate maximum likelihood states and measurements along the trajectory,
we can omit the \ac{EKF} state prediction and state correction.
The propagation of the state covariance depends on the linearization points along the trajectory and thus the choice of maneuvers.


==> chapters/rig.tex <==
\section{Planning Algorithm}\label{sec:planner}
In this section we present the sampling-based information gathering algorithm we use for finding an optimal system identification experiment trajectory.
We rapidly sample the configuration space of the \ac{MAV} by building a graph of polynomial segments.
For every candidate trajectory in the graph we make a prediction about the state and parameter covariance using the \ac{EKF} propagation presented in previous section \ref{sec:propagation}.
Finally, we pick the best trajectory using the D-optimality criterion (\ref{eq:dopt}).

Listing (\ref{lst:algorithm}) describes the full algorithm.
It combines parameter belief propagation as in \ac{RRBT} with \ac{RIG} \cite{Bry2011, Hollinger2014}.
\input{graphics/algorithm}
\subsection{Bidirectional Graph}
For searching the configuration space we build a bidirectional graph of polynomial segments (line \ref{alg:sample} -- \ref{alg:end_connection}).
This allows the \ac{MAV} going forward, backward and circling between nodes.
A belief $n$ labels every possible unique path through that graph.
A belief contains the propagated state covariance matrix, the cost traveled so far, the address of its parent belief and its residing vertex.

The algorithm starts with an initial node which contains an initial state and belief about states and parameters.
It then continuously extends the graph by randomly sampling a vertex and connecting all nearby nodes to the newly sampled one.
Every new connection opens up new possible trajectories through the graph.
We evaluate these by propagating the beliefs at the beginning of the new trajectories along the candidate segments.
Like Achtelik \cite{achtelik2014motion} we \textsc{Sample} uniformly in the differentially flat space of position and yaw $[\posworld~\yaw]^T$.
The first polynomial connection from the nearest to the new vertex locks the new vertices' flat state derivatives.
\begin{align}
\flatstate = \begin{bmatrix}
\posworld^T ~ \velworld^T ~ \accworld^T ~ \jerkworld^T ~ \snapworld^T ~ \yaw ~ \yawdot ~ \yawddot
\end{bmatrix}^T \label{eq:flat_state}
\end{align}%
\textsc{Connect} generates $4D$-polynomial segments with respect to minimum-snap in position and minimum angular velocity in yaw using Richter's optimization \cite{richter2013polynomial}.
We sample the segment time $t$ uniformly for each new connection.
The maximum velocity $v_{max}$ and the euclidean Distance $d$ between the two vertices gives its lower bound.
The maximum budget left within all beliefs at the near vertex determines its upper bound.
We limit the maximum segment time further by a fixed upper time $t_{\textrm{max}} \leq B$ to reduce the search space.
\begin{align}
t \in \left[ \frac{d}{v_{max}}, \max ( \cost{v_{\textrm{near}}.N_{\textrm{open}}}, t_{\textrm{max}} ) \right].
\end{align}%
The segment time fundamentally determines the trajectory shape and thus the parameter observability.

This sampling strategy boils down the high dimensional configuration space of $13$ states and $6$ inputs to $4$ flat states and time.
As described in section \ref{sec:linearization_point} we can recover the nominal states and inputs from the flat state polynomial segments.

Another advantage of sampling in flat polynomial space are quick feasibility checks.
Checking input and state constraints allows meeting hardware and safety constraints.
\textsc{Connect}() tests input and position feasibility of segments applying Mueller's recursive test \cite{muellercomputationally}.
His algorithm rapidly checks a polynomial segment on an upper bound in acceleration and roll and pitch rates as well as box constraints in position.
In addition we check yaw rates and accelerations by evaluating the roots of the appropriate polynomial.
\subsection{Propagation}
Once we connected all neighbors to a new node, we evaluate all new possible path combinations through the graph in the propagation phase (line \ref{alg:search_start} -- \ref{alg:search_end}).
Therefore, we add all open beliefs with a connection to the new vertex to a search queue $Q$.
Then we propagate these beliefs along all outgoing edges which we have not propagated them along, yet.
\textsc{AppendBelief}() decides whether we add the newly generated beliefs to the graph or even on top of the queue, such that we will propagate them even further.

Because a trajectory can revisit older nodes in the graph, different beliefs can traverse one polynomial segment multiple times.
According to Prentice \cite{Prentice2009}, we combine the consecutive \ac{EKF} motion updates (\ref{eq:prior}) and measurement updates (\ref{eq:posterior}) along an edge into a single linear transfer function $\mathcal{S}_{0:T}$ by factoring the covariance.
\begin{align}
\begin{bmatrix}
\cdot & \sigmastate_{T|T} \\
\cdot & \cdot
\end{bmatrix} &=
\begin{bmatrix}
\identity & \sigmastate_{0|0} \\
\zero & \identity
\end{bmatrix}
\star \mathcal{S}_{0:T}.
\end{align}%
We precompute and store $\mathcal{S}_{0:T}$ at every new edge:
\begin{align}
\mathcal{S}_{0:T} &= \mathcal{S}_0 \star \mathcal{S}_1 \star \cdots \star \mathcal{S}_T, &\mathcal{S}_k &= \mathcal{S}_k^C \star \mathcal{S}_k^M .
\end{align}%
The motion update $\mathcal{S}_k^C$ and measurement update $\mathcal{S}_k^M$ are
\begin{align}
\mathcal{S}_k^C &=
\begin{bmatrix}
\systemmat & \processnoisecovdiscrete \\
\zero & \systemmat^T
\end{bmatrix},
&
\mathcal{S}_k^M &=
\begin{bmatrix}
\identity & \zero \\
-\measurementmat^T \measurementnoisecovdiscrete^{-1} \measurementmat & \identity
\end{bmatrix}.
\end{align}%
We interconnect two models using the Redheffer star product:
\begin{align}
&\begin{bmatrix}
\mat{A} & \mat{B}\\
\mat{C} & \mat{D}
\end{bmatrix}
\star
\begin{bmatrix}
\mat{W} & \mat{X}\\
\mat{Y} & \mat{Z}
\end{bmatrix}
= \\
&\begin{bmatrix}
\mat{W} (\identity-\mat{B}\mat{Y}) ^{-1} \mat{A} & \mat{X} + \mat{W} (\identity-\mat{B}\mat{Y})^{-1} \mat{B}\mat{Z} \\
\mat{C} + \mat{D}(\identity-\mat{Y}\mat{B})^{-1}\mat{Y}\mat{A} & \mat{D}(\identity - \mat{Y}\mat{B})^{-1} \mat{Z}
\end{bmatrix}.
\end{align}%
This one-step propagation reduces the computational complexity of \textsc{Propagate}().

\subsection{Pruning}
Still, a major bottleneck of the algorithm is the uniform cost search.
Without pruning, the search explores every new possible path segment combination every time we add a new vertex to the graph.
As the number of interconnections grows the planner soon comes to halt.
We apply belief pruning, trading off optimality guarantees for computational feasibility.

\textsc{AppendBelief}() controls whether we add a new belief to the graph during the propagation phase.
On the one hand it checks whether a belief's cost remains within the budget. If it does, we consider it open.
If it is out of budget, it is either considered as closed or discarded in case the budget is overly exceeded.
On the other hand it checks whether the new belief is either dominated by any other belief already at the target vertex or if it is dominating any other belief itself.
We prune dominated beliefs.
We consider a belief better than another if it has smaller cost, total state uncertainty  $\sigmastate$ and parameter uncertainty $\sigmaparameter$.
\begin{align}
&n_a < n_b \Leftrightarrow \label{eq:compare} \\
&\cost{n_a} < \cost{n_b} \wedge n_a.\sigmastate < n_b.\sigmastate \wedge n_a.\sigmaparameter < n.b.\sigmaparameter \nonumber
\end{align}%
We compare covariance matrices using the D-optimality criterion (\ref{eq:dopt}).
Because the objective function is submodular the pruning (\ref{eq:compare}) causes loss of optimality \cite{Hollinger2014}.
We add the complete state covariance $\sigmastate$ to the comparison (\ref{eq:compare}), since a converged state can have positive influence on a parameter update.


==> chapters/steering.tex <==
\section{Connection Generation}\label{sec:steering}

\subsection{Polynomial Sampling}
Flat state sample + time, polynomial constraint minimum snap optimization,

\subsection{Recursive Feasibility Check}
input and state feasibility check

\subsection{Full State Recovery}
Approximately the rotor speeds, attitude and angular velocity can be derived from the flat states and its derivatives following Mellinger \cite{mellinger2011minimum}.

\noindent From the trajectories we have the state in world coordinates.
\begin{align}
\mathbf{x}_f &= \begin{bmatrix}
\mathbf{p}^T & \mathbf{v}^T & \mathbf{a}^T & \mathbf{j}^T & \mathbf{s}^T & \psi & \dot{\psi} & \ddot{\psi}
\end{bmatrix}^T
\end{align}%
The full attitude $\mathbf{q}$ is described as
\begin{align}
\mathbf{z}_B &= \frac{\mathbf{t}}{|\mathbf{t}|}, & \mathbf{t} = \mathbf{a} + \begin{bmatrix}
0 & 0 & g
\end{bmatrix}^T, \\
\mathbf{y}_B &= \frac{\mathbf{z}_B \times \mathbf{x}_C}{||\mathbf{z}_B \times \mathbf{x}_C||}, & \mathbf{x}_C = \begin{bmatrix}
\cos \psi & \sin \psi & 0
\end{bmatrix}^T, \\
\mathbf{x}_B &= \mathbf{y}_B \times \mathbf{z}_B, \\
\mathbf{C}(\mathbf{q}) &= \begin{bmatrix}
\mathbf{x}_B & \mathbf{y}_B & \mathbf{z}_B
\end{bmatrix}, & ||\mathbf{z}_B \times \mathbf{x}_C|| \neq 0.
\end{align}%
The angular velocity $\boldsymbol{\omega}$ is
\begin{align}
\mathbf{h}_\omega & = \frac{1}{|\mathbf{t}|} \left( \mathbf{j} - \left( \mathbf{z}_B^T \cdot \mathbf{j} \right) \mathbf{z}_B \right), \\
\omega_1 &= - \mathbf{h}_\omega^T \cdot \mathbf{y}_B ,\\
\omega_2 &= \mathbf{h}_\omega^T \cdot \mathbf{x}_B ,\\
\omega_3 &= \dot \psi \cdot \mathbf{z}_W^T \cdot \mathbf{z}_B .
\end{align}%
The angular acceleration $\boldsymbol{\alpha}$ is
\begin{align}
\mathbf{h}_\alpha &=  \left( \frac{1}{|\mathbf{t}|} \left( \mathbf{s} - \left( \mathbf{z}_B^T \cdot \mathbf{s} \right) \mathbf{z}_B \right) - 2  \left(\boldsymbol{\omega} \times \mathbf{z}_B \right) - \boldsymbol{\omega} \times \left( \boldsymbol{\omega} \times \mathbf{z}_B \right) + \mathbf{z}_B^T \left( \boldsymbol{\omega} \times \left( \boldsymbol{\omega} \times \mathbf{z}_B \right) \right) \mathbf{z}_B    \right), \\
\alpha_1 &= -\mathbf{h}_\alpha^T \cdot \mathbf{y}_B, \\
\alpha_2 &= \mathbf{h}_\alpha \cdot \mathbf{x}_B, \\
\alpha_3 &= \ddot \psi \mathbf{z}_W^T \cdot \mathbf{z}_B.
\end{align}%
Finally, a linear mapping $\mathbf{A}$ between thrust $T$ and torques $\boldsymbol{\tau}$ and rotor speeds $\mathbf{n}$ exists, which allows us calculating the rotor speeds.
\begin{align}
\begin{bmatrix}
 \boldsymbol{\tau} \\ T 
\end{bmatrix} &= \mathbf{K} \cdot \mathbf{A} \cdot \mathbf{n}^2, \\
\boldsymbol{\tau} &= \mathbf{J} \boldsymbol{\alpha} + \boldsymbol{\omega} \times \mathbf{J} \boldsymbol{\omega}, \\
T &= m |\mathbf{t}|.
\end{align}%
For a hexacopter we get
\begin{align}
\mathbf{A} &= \begin{bmatrix}
s & 1 & s & -s & -1 & -s \\
-c & 0 & c & c & 0 & -c \\
-1 & 1 & -1 & 1 & -1 & 1 \\
1 & 1 & 1 & 1 & 1 & 1
\end{bmatrix}, \\
\mathbf{K} &= \mathrm{diag} \left( \begin{bmatrix}
l \kthr  & l \kthr & \kthr \kmom & \kthr
\end{bmatrix} \right),
\end{align}%
where $s = \sin (\SI{30}{\degree})$, $c = \cos (\SI{30}{\degree})$ and $l$ is the rotor arm length. The squared rotor speeds, which are required for linearization, can now be obtained from known quantities.
\begin{align}
\mathbf{n}^2 &=  A^\dagger \cdot K^{-1} \cdot \begin{bmatrix}
 \boldsymbol{\tau} \\ T 
\end{bmatrix}
\end{align}%

==> graphics/tab_uncertainty.tex <==
\begin{table}[b]
\caption{Final parameter uncertainty in $100$ simulated calibrations.}
\begin{center}
\label{tab:uncertainty}
\begin{tabular}{llccccc}
\toprule
Planner                           & MEAN D-Optimality                  & STDEV D-Optimality              \\
\midrule
RAND                              &                                    &                                 \\
OUR                               &                                    &                                 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

